Utilizing Redundancy in Cost Functions for Resilience in Distributed Optimization and Learning

This paper considers the problem of resilient distributed optimization and stochastic machine learning in a server-based architecture. The system comprises a server and multiple agents, where each agent has a local cost function. The agents collaborate with the server to find a minimum of their aggregate cost functions. We consider the case when some of the agents may be asynchronous and/or Byzantine faulty. In this case, the classical algorithm of distributed gradient descent (DGD) is rendered ineffective. Our goal is to design techniques improving the efficacy of DGD with asynchrony and Byzantine failures. To do so, we start by proposing a way to model the agents' cost functions by the generic notion of $(f, \,r; \epsilon)$-redundancy where $f$ and $r$ are the parameters of Byzantine failures and asynchrony, respectively, and $\epsilon$ characterizes the closeness between agents' cost functions. This allows us to quantify the level of redundancy present amongst the agents' cost functions, for any given distributed optimization problem. We demonstrate, both theoretically and empirically, the merits of our proposed redundancy model in improving the robustness of DGD against asynchronous and Byzantine agents, and their extensions to distributed stochastic gradient descent (D-SGD) for robust distributed machine learning with asynchronous and Byzantine agents.

==> stochastic.old.tex <==
\section{Resilient stochastic machine learning}
\label{sec:stochastic}

As discussed in Section~\ref{sub:learning}, resilient distributed machine learning problems can be formulated in the same forms of resilient distributed optimization problems, but the stochastic method D-SGD is more commonly used than DGD. In this section, we show how to utilize $(f,r;\epsilon)$-redundancy to achieve resilient distributed machine learning.

We first briefly revisit the computation of stochastic gradients in a distributed machine learning system. To compute a stochastic gradient in iteration $t$, a (non-faulty) agent $i$ samples $k$ i.i.d. data points $z_{i_1}^t,...,z_{i_k}^t$ from the distribution $\mathcal{D}_i$ and computes
\begin{equation}
    \textstyle g_i^t=\frac{1}{k}\sum_{i=1}^k\nabla\ell(w^t, z_{i_j}^t),
    \label{eqn:def-g-i-t}
\end{equation}
where $k$ is referred to as the \textit{batch size} of the training procedure.

We will also use the following notations in this section. Suppose faulty agents (if any) in the system are \textit{fixed} during a certain execution. For each non-faulty agent $i$, let $\z_i^t=\left\{z_{i_1}^t,...,z_{i_k}^t\right\}$ denote the collection of $k$ i.i.d. data points sampled by agent $i$ at iteration $t$. Now for each agent $i$ and iteration $t$, we define a random variable 
\begin{equation}
    \zeta_i^t=\begin{cases}
        \z_i^t, & \textrm{ agent $i$ is non-faulty}, \\
        g_i^t, & \textrm{ agent $i$ is faulty}.
    \end{cases}
    \label{eqn:zeta-i-t-cge}
\end{equation}
Recall that $g_i^t$ can be an arbitrary $d$-dimensional random variable for each Byzantine faulty agent $i$. For each iteration $t$, let $\zeta^t=\left\{\zeta_i^t,\,i=1,...,n\right\}$, and let $\E_t$ denote the expectation with respect to the collective random variables $\zeta^0,...,\zeta^t$, given the initial estimate $x^0$. Specifically, 
\begin{equation}
    \E_t(\cdot)=\E_{\zeta^0,...,\zeta^t}(\cdot), ~\forall t\geq0.
\end{equation}

\subsection{Byzantine learning}

Consider Problem BS in Table~\ref{tab:problems}. Specifically, the resilient machine learning problem where there are 0 asynchronous agents and up to $r$ Byzantine agents. Due to the existence of Byzantine agents, the goal is to solve \eqref{eqn:goal-ft}. Suppose $\H\subset[n]$ is a subset of non-faulty agents with $\mnorm{\H}=n-f$. We make the same Assumptions~\ref{assum:lipschitz} and \ref{assum:strongly-convex-ft}. The existence of a solution to \eqref{eqn:goal-ft} is guaranteed by \eqref{eqn:existence-ft}. We also need an extra assumption to bound the variance of stochastic gradients from non-faulty agents. 
\begin{assumption}
     \label{assum:bound-grad-ft}
     For each non-faulty agent $i$, assume that the variance of $g_i^t$ is bounded. Specifically, there exists a finite real value $\sigma$ such that for all non-faulty agent $i$,
     \begin{equation}
          \E_{\zeta_i^t}\norm{g_i^t-\E_{\zeta_i^t}\left(g_i^t\right)}^2\leq\sigma^2.
          \label{eqn:assum-bound-var-ft}
     \end{equation}
\end{assumption}

Recall \eqref{eqn:update} in \textbf{Step 2} of our Algorithm~\ref{alg}. We define the gradient aggregation rule for Problem BS to be
\begin{align}
    \textstyle\mathsf{GradAgg}\left(g_j^t|j\in S^t;n,f,0\right)
    =\mathsf{GradFilter}\left(g_j^t|j\in[n];n,f\right)
    \label{eqn:aggregation-rule-ft}
\end{align}
for every iteration $t$. Note that $r=0$ since there is no asynchronous agent in this problem.

We define a \textit{fault-tolerance margin} $\alpha$ that determines the fraction of faulty agents $f/n$ that can be tolerated by our algorithm for given parameters $\mu$ and $\lambda$. Specifically,
\begin{align}
    \alpha = \frac{\lambda}{\lambda+2\mu}-\frac{f}{n}.
    \label{eqn:def-alpha-ft}
\end{align}
We also define a parameter
\begin{align}
    \overline{\eta} = \left(\frac{2(\lambda+2\mu)n}{\left( (n-f)^2+4n^2\epsilon^2 \right)\mu^2}\right)\alpha.
    \label{eqn:def-eta-bar-ft}
\end{align}
that determines the value of step size in \eqref{eqn:update}. We have the following result regarding the convergence speed of Algorithm~\ref{alg}.

\begin{theorem}
    \label{thm:cge}
    Consider Algorithm~\ref{alg} with CGE gradient filter. Suppose Assumptions~\ref{assum:lipschitz}, \ref{assum:strongly-convex-ft}, and \ref{assum:bound-grad-ft} hold true, the expected cost functions of non-faulty functions satisfy $(2f,\epsilon)$-redundancy, $\alpha>0$ and step size in \eqref{eqn:update} $\eta_t=\eta>0$ for all $t$. Let
    \begin{align}
        \M &= 4n^2(n-f)^2\eta^2\mu^2\epsilon^2 +\left(2f+\frac{f\sigma}{2n\mu\epsilon}+(n-f)^2\eta\mu\right)^2 \nonumber \\
        &\qquad+ (n-f)^2\eta^2\sigma^2.
        \label{eqn:def-m}
    \end{align}
    If $\eta<\overline{\eta}$, the following holds true:
    \begin{itemize}
        \item The value of 
        \begin{align}
            \rho &= 1-\left( (n-f)^2+4n^2\epsilon^2 \right)\mu^2\eta\left(\overline{\eta}-\eta\right)
            \label{eqn:def-rho}
        \end{align}
        satisfies $0<\rho<1$, and 
        \item Given the initial estimate $w^0$ arbitrarily chosen from $\R^d$, for all $t\geq0$,
        \begin{align}
            \E_{t}\norm{w^{t+1}-w_\H}^2&\leq\rho^{t+1}\norm{w^0-w_\H}^2 + \left(\frac{1-\rho^{t+1}}{1-\rho}\right)\M.
            \label{eqn:expectation-bound-1}
        \end{align}
    \end{itemize}
\end{theorem}

\subsection{Asynchronous learning}
\label{sub:async-learning}

Consider Problem CS in Table~\ref{tab:problems}. Specifically, the resilient machine learning problem where there are up to $r$ asynchronous agents and 0 Byzantine agents. The goal is to solve \eqref{eqn:goal}. We make the Assumptions~\ref{assum:lipschitz} and \ref{assum:strongly-convex}. We assume \eqref{eqn:existence-exact}, the existence of a solution. We also need an extra assumption to bound the variance of stochastic gradients.

\begin{assumption}
     \label{assum:bound-grad}
     For each agent $i$, assume that the variance of $g_i^t$ is bounded. Specifically, there exists a finite real value $\sigma$ such that for every agent $i$,
     \begin{equation}
          \E_{\zeta_i^t}\norm{g_i^t-\E_{\zeta_i^t}\left(g_i^t\right)}^2\leq\sigma^2.
          \label{eqn:assum-bound-var}
     \end{equation}
\end{assumption}

Recall \eqref{eqn:update} in \textbf{Step 2} of our Algorithm~\ref{alg}. We define the gradient aggregation rule for Problem CS to be \eqref{eqn:aggregation-rule}. Note that $f=0$ in this problem.

We define a value $\alpha$ that determines the fraction of stragglers $r/n$ that can be tolerated by our algorithm for given parameters $\mu$ and $\gamma$. Specifically,
\begin{align}
    \alpha = \frac{\gamma}{\mu}-\frac{r}{n}.
    \label{eqn:def-alpha}
\end{align}
We also define a parameter
\begin{align}
    \overline{\eta} = \frac{2n}{\left((n-r)^2+4n^2\epsilon^2\right)\mu}\alpha.
    \label{eqn:def-eta-bar}
\end{align}
that determines the value of step size in \eqref{eqn:update}.

\begin{theorem}
    \label{thm:approx-sgd}
    Consider Algorithm~\ref{alg} with stochastic updates. Suppose Assumptions~\ref{assum:lipschitz}, \ref{assum:strongly-convex}, and \ref{assum:bound-grad} hold true, the expected cost functions of the agents in the system satisfy $(r,\epsilon)$-redundancy, $\alpha>0$ and step size in \eqref{eqn:update} $\eta_t=\eta>0$ for all $t$. Let
    \begin{align}
        \M &= 4n^2(n-r)^2\eta^2\mu^2\epsilon^2+(n-r)^2\eta^2\sigma^2 \nonumber \\
        &\qquad+ \left(r + (n-r)^2\eta\mu\right)^2.
        \label{eqn:def-m}
    \end{align}
    If $\eta<\overline{\eta}$, the following holds true:
    \begin{itemize}
        \item The value of 
        \begin{align}
            \rho &= 1-\left((n-r)^2+4n^2\epsilon^2\right)\mu^2\eta\left(\overline{\eta}-\eta\right)
            \label{eqn:def-rho}
        \end{align}
        satisfies $0<\rho<1$, and 
        \item Given the initial estimate $x^0$ arbitrarily chosen from $\R^d$, for all $t\geq0$,
        \begin{align}
            \E_{t}\norm{x^{t+1}-x^*}^2&\leq\rho^{t+1}\norm{x^0-x^*}^2 + \left(\frac{1-\rho^{t+1}}{1-\rho}\right)\M.
            \label{eqn:expectation-bound-1}
        \end{align}
    \end{itemize}
\end{theorem}

\subsection{Asynchronous Byzantine learning}
\label{sub:async-ft-learning}
Finally, consider Problem DS in Table~\ref{tab:problems}. Specifically, the resilient machine learning problem where there are up to $r$ asynchronous agents and up to $f$ Byzantine agents, for which overlapping is possible. Due to the existence of Byzantine agents, the goal here is to solve \eqref{eqn:goal-ft}. Suppose $\H\subset[n]$ is a subset of non-faulty agents with $\mnorm{\H}=n-f$. We make the same Assumptions~\ref{assum:lipschitz}, \ref{assum:strongly-convex-ft}, \ref{assum:bound-grad-ft}, and existence of solution \eqref{eqn:existence-ft}. 

Recall \eqref{eqn:update} in \textbf{Step 2} of our Algorithm~\ref{alg}. We define the gradient aggregation rule for Problem DS to be \eqref{eqn:aggregation-rule-async-ft}. 

We define a value $\alpha$ that determines the fraction of stragglers $r/n$ that can be tolerated by our algorithm for given parameters $\mu$ and $\gamma$. Specifically,
\begin{align}
    \alpha = \frac{\gamma}{2\mu}\cdot\left(1-\frac{f-r}{n-r}\right)+\frac{f+r}{n-r}.
    \label{eqn:def-alpha-cge}
\end{align}
We define a parameter
\begin{align}
    \overline{\eta} = \frac{4(n-r)}{\left( (n-r-f)^2+4(n-r)^2\epsilon^2 \right)\mu}\alpha.
    \label{eqn:def-eta-bar-cge}
\end{align}
that determines the value of step size in \eqref{eqn:update}.

\begin{theorem}
    \label{thm:approx-sgd-cge}
    Consider Algorithm~\ref{alg} with stochastic updates. Suppose Assumptions~\ref{assum:lipschitz}, \ref{assum:strongly-convex}, and \ref{assum:bound-grad} hold true, the expected cost functions of the agents in the system satisfy $(r,\epsilon)$-redundancy, $\alpha>0$, step size in \eqref{eqn:update} $\eta_t=\eta>0$ for all $t$, and $n\geq 2f+r/2$. Let
    \begin{align}
        \M =& 4(n-r)^2(n-r-f)^2\eta^2\mu^2\epsilon^2 \nonumber \\
        &+\left(2(f+r)+\frac{(f+r)\sigma}{2(n-r)\mu\epsilon}+(n-r-f)^2\eta\mu\right)^2 \nonumber \\
        &+ (n-r-f)^2\eta^2\sigma^2.
        \label{eqn:def-m-cge}
    \end{align}
    If $\eta<\overline{\eta}$, the following holds true:
    \begin{itemize}
        \item The value of 
        \begin{align}
            \rho &= 1 - \left( (n-r-f)^2+4(n-r)^2\epsilon^2 \right)\mu^2\eta\left(\overline{\eta}-\eta\right).
            \label{eqn:def-rho-cge}
        \end{align}
        satisfies $0<\rho<1$, and 
        \item Given the initial estimate $x^0$ arbitrarily chosen from $\R^d$, for all $t\geq0$,
        \begin{align}
            \E_{t}\norm{x^{t+1}-x_\H}^2&\leq\rho^{t+1}\norm{x^0-x_\H}^2 + \left(\frac{1-\rho^{t+1}}{1-\rho}\right)\M.
            \label{eqn:expectation-bound-1-cge}
        \end{align}
    \end{itemize}
\end{theorem}

